AiOS: All-in-One-Stage Expressive Human Pose and Shape Estimation

Expressive human pose and shape estimation (a.k.a. 3D whole-body mesh recovery) involves the human body, hand, and expression estimation. Most existing methods have tackled this task in a two-stage manner, first detecting the human body part with an off-the-shelf detection model and inferring the different human body parts individually. Despite the impressive results achieved, these methods suffer from 1) loss of valuable contextual information via cropping, 2) introducing distractions, and 3) lacking inter-association among different persons and body parts, inevitably causing performance degradation, especially for crowded scenes. To address these issues, we introduce a novel all-in-one-stage framework, AiOS, for multiple expressive human pose and shape recovery without an additional human detection step. Specifically, our method is built upon DETR, which treats multi-person whole-body mesh recovery task as a progressive set prediction problem with various sequential detection. We devise the decoder tokens and extend them to our task. Specifically, we first employ a human token to probe a human location in the image and encode global features for each instance, which provides a coarse location for the later transformer block. Then, we introduce a joint-related token to probe the human joint in the image and encoder a fine-grained local feature, which collaborates with the global feature to regress the whole-body mesh. This straightforward but effective model outperforms previous state-of-the-art methods by a 9% reduction in NMVE on AGORA, a 30% reduction in PVE on EHF, a 10% reduction in PVE on ARCTIC, and a 3% reduction in PVE on EgoBody.

==> sections/D_experiment_2.tex <==
\clearpage
% \input{tables/agora_smpl_test}
\section{Comparison with Existing Methods on AGORA SMPL} \label{sec_3}

As the first one-stage method in the Expressive Human Pose and Shape Estimation (EHPS), we cannot locate relevant one-stage work for a fair comparison. Therefore, in this section, similar to Hand4Whole~\cite{hand4whole}, we compare the results of our body part with existing body-only methods, which can be broadly categorized into top-down methods~\cite{hmr, pymaf,pare,cliff, li2020hybrik,propose,pliks, niki} and one-stage methods~\cite{romp,bev}, on the AGORA SMPL test set.
Specifically, we downsample the SMPL-X mesh estimated by AiOS to the SMPL~\cite{smpl} mesh using official tools~\cite{smplx} and then measure MVE and NMVE. We use the J-regressor from SMPL to regress joints from the downsampled SMPL mesh to measure NMJE and MPJPE.

We first compare AiOS with one-stage methods, ROMP~\cite{romp} and BEV~\cite{bev}. As we mentioned in the main paper, both ROMP and BEV perceive the position of a human from the body center heatmap and sample features from the SMPL map based on the perceived body center to perform the regression of SMPL parameters. Despite the impressive results achieved by ROMP and BEV, we believe that representing the entire human body using only one center is inadequate. As shown in \Tab~\ref{tab:agora_smpl_test}, AiOS, designed specifically for expressive human pose and shape estimation, significantly outperforms ROMP and BEV, with a notable improvement in NMVE of 43\% (from 108.3 mm to 61.2 mm) and a NMJE enhancement of 40\% (from 113.2 mm to 68.0 mm). It is worth noting that we do not deliberately fine-tune our model exclusively on AGORA. In \Fig\ref{fig:sup_romp}, we compare the visualizations of AiOS with ROMP and BEV.   
While ROMP and BEV can achieve decent results for body reconstruction in multi-person scenarios, they are limited by the constraints of the SMPL~\cite{smpl} model, preventing them from reconstructing detailed hand gestures and facial expressions.



We also compare AiOS with the state-of-the-art top-down methods~\cite{hmr, pymaf, pare, cliff, li2020hybrik, propose,pliks, niki}. Since there are no publicly available annotations for the AGORA test set, existing top-down methods initially employ an off-the-shelf detection model to detect humans, and then they utilize their proposed methods to reconstruct the SMPL model. Once again, AiOS demonstrates a significant lead over existing state-of-the-art algorithms, even with a higher recall.






\clearpage



\begin{figure*}[h]
    \centering
  \includegraphics[width=1\linewidth]{pictures/romp_supp.pdf}
    \caption{\textbf{Additional visual comparisons of existing one-stage methods on the Internet data.} 
    The first column is the input images, and they are downloaded from the internet. The second column is the visualization results of ROMP~\cite{romp}, the third column shows the visualization results of BEV~\cite{bev}, and the last column illustrates our visualization results.
    }
    \label{fig:sup_romp}
    % \vspace{-10pt}
\end{figure*}

\clearpage


==> sections/G_Implementation.tex <==
\noindent\textbf{Training set.} 
AiOS is trained using the multi-person datasets AGORA~\cite{agora}, BEDLAM~\cite{bedlam}, and COCO~\cite{coco}, and single-person datasets UBody~\cite{osx}, ARCTIC~\cite{arctic}, and EgoBody~\cite{egobody}. Among them, AGORA and BEDLAM are the synthetic datasets~\cite{agora, bedlam}, which provide high-quality SMPL-X annotations and various crowded scenarios that are difficult to obtain from the real world.

\input{tables/agora_test}
\input{tables/agora_smpl_test}
% \input{tables/bedlam}
\noindent\textbf{Implementation details.}


The training is conducted on 16 V100 GPUs, with a total batch size of 32. 


During the training stage, the shorter side of the input image is resized to 800, and the maximum size is restricted to 1333. We also adopt several other data augmentations to enhance the diversity and adaptability of the model, such as color jittering, random horizontal flipping, and instance cropping. 

We initialize AiOS's backbone, encoder, and part of the decoder from a weight trained on COCO human pose estimation, provided by ED-Pose ~\cite{edpose}. We use Adam optimizer with a step learning rate for training. We first train our model for 60 epochs with an initial learning rate $1 \times 10^{-4}$ and drop at the 50th epoch on AGORA, BEDLAM, and COCO. We finetune it for 50 epochs with $1 \times 10^{-5}$ initial learning rate and drop at the 25th epoch on all train datasets. 


\noindent\textbf{Test set.} 
We use AGORA~\cite{agora} for most of our quantitative comparison with other methods, and it is evaluated by the official evaluation server. We also report EHF~\cite{smplx}, Egobody~\cite{egobody}, UBody~\cite{osx} and ARCTIC~\cite{arctic} for our performance on real-life single-person datasets, and we match the ground truth 2D keypoints with our predicted keypoints and then report all metrics. 





\noindent
\textbf{Evaluation metrics.}
Following the previous EHPS methods~\cite{hand4whole, osx, smplerx}, we report the MPVPE (mean per-vertex position error) and PA-MPVPE (Procrutes Aligned per-vertex position error) across all benchmarks. In AGORA
Leaderboard, we report MVE (mean vertex error), MPJPE (mean per-joint position error) for pure SMPL-X regression accuracy; F Score, precision, recall for detection accuracy; NMVE (normalized mean vertex error) and NMJE (normalized mean joint error) that considered regression accuracy with detection accuracy.  All reconstruction errors are reported in millimeters (mm).

==> tables/ablation_1.tex <==
\begin{table}[t]
\centering
\resizebox{0.5\textwidth}{!}{
    \begin{tabular}{lcccccc}
    \toprule
    & 
    \multicolumn{3}{c}{PA-PVE$\downarrow$ (\emph{mm})} &
    \multicolumn{3}{c}{PVE$\downarrow$ (\emph{mm})} \\
    
    \cmidrule(lr){2-4} \cmidrule(lr){5-7} 
    
    Method &
    All & Hands & Face &
    All & Hands & Face \\
    
    \midrule

    Native AiOS & 
    \textbf{34.0} & \underline{12.8} & \textbf{3.8}& \textbf{45.4} & \underline{44.1} & \textbf{16.9}\\
    AiOS & 
    \textbf{34.0} & \underline{12.8} & \textbf{3.8}& \textbf{45.4} & \underline{44.1} & \textbf{16.9}\\    
    \bottomrule
    \end{tabular}
}
\vspace{-2mm}
\caption{\textbf{Ablation study 1}. 
xxx
}
\label{tab:abl1}
\end{table}

==> tables/ablation_3.tex <==
\begin{table}[t]
\centering
\resizebox{0.5\textwidth}{!}{
    \begin{tabular}{lcccccc}
    \toprule

     &
    All & Hands & Face &
    All & Hands & Face \\
    
    \midrule



    baseline1& 
    42.7 & 7.4 & 4.2& 55.7 & 39.8 & 25.1\\ 
     baseline2 & 
    40.3& 7.2 & 4.2& 51.8 & 38.0 & 23.8\\ 
    Ours& 
   39.9 & 7.2 & 4.1&  50.5 & 37.4 & 23.3\\ 
    \bottomrule
    \end{tabular}
}
\vspace{-2mm}
\caption{\textbf{The association between human body part}. 
xxx
}
\label{tab:abl3}
\end{table}

==> tables/ablation_4.tex <==
\begin{table}[t]
\centering
\resizebox{0.5\textwidth}{!}{
    \begin{tabular}{lcccccc}
    \toprule

     &
    All & Hands & Face &
    All & Hands & Face \\
    
    \midrule



    baseline1& 
    42.7 & 7.4 & 4.2& 55.7 & 39.8 & 25.1\\ 
     baseline2 & 
    40.3& 7.2 & 4.2& 51.8 & 38.0 & 23.8\\ 
    Ours& 
   39.9 & 7.2 & 4.1&  50.5 & 37.4 & 23.3\\ 
    \bottomrule
    \end{tabular}
}
\vspace{-2mm}
\caption{\textbf{Ablation Studies}. 
}
\label{tab:abl3}
\end{table}


